Robust asymptotic insurance-finance arbitrage

In most cases, insurance contracts are linked to the financial markets, such as through interest rates or equity-linked insurance products. To motivate an evaluation rule in these hybrid markets, Artzner et al. (2022) introduced the notion of insurance-finance arbitrage. In this paper we extend their setting by incorporating model uncertainty. To this end, we allow statistical uncertainty in the underlying dynamics to be represented by a set of priors $\mathscr{P}$. Within this framework we introduce the notion of robust asymptotic insurance-finance arbitrage and characterize the absence of such strategies in terms of the concept of ${Q}\mathscr{P}$-evaluations. This is a nonlinear two-step evaluation which guarantees no robust asymptotic insurance-finance arbitrage. Moreover, the ${Q}\mathscr{P}$-evaluation dominates all two-step evaluations as long as we agree on the set of priors $\mathscr{P}$ which shows that those two-step evaluations do not allow for robust asymptotic insurance-finance arbitrages. Furthermore, we introduce a doubly stochastic model under uncertainty for surrender and survival. In this setting, we describe conditional dependence by means of copulas and illustrate how the ${Q}\mathscr{P}$-evaluation can be used for the pricing of hybrid insurance products.

==> commands.tex <==

%\usepackage{showframe} %nice way to find out the layout of the paper

\usepackage{geometry}
\geometry{a4paper,hcentering,vcentering,outer=2.8cm,top=3cm}

% Bibliography Style
% \usepackage[numbers]{tsnatbib}
% Alternative:
\usepackage[round,comma]{natbib}                %works better with hyperref

\usepackage{enumerate}
\usepackage{mathabx}


% Maths:
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{dsfont}

\usepackage{nicefrac}
\usepackage{booktabs}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage{mathtools}



%for bold math symbols
%\usepackage{stmaryrd}    % \llbracket
% Could be replaced by \usepackage{marvosym} if Font Declaration problems appear
% Double Brackets
%\ldbrack (mathabx) and \llbracket (stmaryrd)

%#\usepackage[percent]{overpic}
% Zum Beschriften von Bildern. Bsp:
% \begin{overpic}[scale = 0.6,grid,tics=5]{graphics/fig18neu.eps}
% \put(25,60){$\sum_{i=1}^10 x_i$}
% \end{overpic}

% My definitions
\newcommand{\ccA}{{\mathscr A}}\newcommand{\cA}{{\mathcal A}}
\newcommand{\ccB}{{\mathscr B}}\newcommand{\cB}{{\mathcal B}}
\newcommand{\ccC}{{\mathscr C}}\newcommand{\cC}{{\mathcal C}}
\newcommand{\ccD}{{\mathscr D}}\newcommand{\cD}{{\mathcal D}}
\newcommand{\ccE}{{\mathscr E}}\newcommand{\cE}{{\mathcal E}}
\newcommand{\ccF}{{\mathscr F}}\newcommand{\cF}{{\mathcal F}}
\newcommand{\ccG}{{\mathscr G}}\newcommand{\cG}{{\mathcal G}}
\newcommand{\ccH}{{\mathscr H}}\newcommand{\cH}{{\mathcal H}}
\newcommand{\ccI}{{\mathscr I}}\newcommand{\cI}{{\mathcal I}}
\newcommand{\ccJ}{{\mathscr J}}\newcommand{\cJ}{{\mathcal J}}
\newcommand{\ccK}{{\mathscr K}}\newcommand{\cK}{{\mathcal K}}
\newcommand{\ccL}{{\mathscr L}}\newcommand{\cL}{{\mathcal L}}
\newcommand{\ccM}{{\mathscr M}}\newcommand{\cM}{{\mathcal M}}
\newcommand{\ccN}{{\mathscr N}}\newcommand{\cN}{{\mathcal N}}
\newcommand{\ccO}{{\mathscr O}}\newcommand{\cO}{{\mathcal O}}
\newcommand{\ccP}{{\mathscr P}}\newcommand{\cP}{{\mathcal P}}
\newcommand{\ccQ}{{\mathscr Q}}\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\ccR}{{\mathscr R}}\newcommand{\cR}{{\mathcal R}}
\newcommand{\ccS}{{\mathscr S}}\newcommand{\cS}{{\mathcal S}}
\newcommand{\ccT}{{\mathscr T}}\newcommand{\cT}{{\mathcal T}}
\newcommand{\ccU}{{\mathscr U}}\newcommand{\cU}{{\mathcal U}}
\newcommand{\ccV}{{\mathscr V}}\newcommand{\cV}{{\mathcal V}}
\newcommand{\ccW}{{\mathscr W}}\newcommand{\cW}{{\mathcal W}}
\newcommand{\ccX}{{\mathscr X}}\newcommand{\cX}{{\mathcal X}}
\newcommand{\ccY}{{\mathscr Y}}\newcommand{\cY}{{\mathcal Y}}
\newcommand{\ccZ}{{\mathscr Z}}\newcommand{\cZ}{{\mathcal Z}}

% bold: have a look at ams short-guide!
\newcommand{\blambda}{{\boldsymbol \lambda}}
\newcommand{\bxi}{{\boldsymbol \xi}}
\newcommand{\bpsi}{{\boldsymbol \psi}}
\newcommand{\bphi}{{\boldsymbol \phi}}
\newcommand{\bSigma}{{\boldsymbol \Sigma}} %{\mbox{\boldmath$\Sigma$}}
\newcommand{\bsigma}{{\boldsymbol \sigma}}
\newcommand{\balpha}{{\boldsymbol \alpha}}
\newcommand{\btheta}{{\boldsymbol \theta}}
\newcommand{\bLambda}{{\boldsymbol \Lambda}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\be}{\bm{e}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bq}{\bm{q}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bx}{\bm{x}}
\newcommand{\bX}{\bm{X}}
\newcommand{\by}{\bm{y}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}

\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\TTr}{Tr}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\oput}{put}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\corr}{Corr}

\newcommand{\VaR}{\operatorname{VaR}}
\newcommand{\ES}{\operatorname{ES}}
\newcommand{\EDF}{\operatorname{EDF}}
\newcommand{\cov}{\operatorname{Cov}}
\newcommand{\sd}{\operatorname{sd}}


\newcommand{\Ind}{{\mathds 1}}
\newcommand{\ind}[1]{\Ind_{\{#1\}}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\restr}{\mathbf{\kern0.3ex%\vert\kern-0.5ex
 \vert\kern-0.3ex}\backprime\kern0.3ex}
\newcommand{\abs}[1]{|#1|}
\newcommand{\half}{\ ^1\mkern -3mu/ _2\ }
\newcommand{\threehalf}{\ ^3\mkern -3mu/ _2\ }
\newcommand{\norm}[1]{\|#1\|}

\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}

%Caligraphic letter
\renewcommand{\cF}{\ccF}
\renewcommand{\cG}{\ccG}
\renewcommand{\cH}{\ccH}


% Now we define the environments
%\theoremstyle{theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}      %[section]
\newtheorem{lemma}[theorem]{Lemma}              %[section]
\newtheorem{hypothesis}[theorem]{Hypothesis}  %[section]
\newtheorem{proposition}[theorem]{Proposition}  %[section]


\theoremstyle{definition}
\newtheorem{example}[theorem]{Example} %[section]
\newtheorem{definition}[theorem]{Definition} %[section]
\newtheorem{remark}[theorem]{Remark}%[section]
\newtheorem{assumption}[theorem]{Assumption}%[section]


\usepackage[backgroundcolor=white,bordercolor=orange]{todonotes}


\usepackage[colorlinks,urlcolor=red,citecolor=blue,linkcolor=red]{hyperref}

% Format of the text

% Do not forget to have
% \renewcommand{\P}{\mathbb{P}}
% after begin document !



\newcommand*{\medcap}{\mathbin{\scalebox{0.9}{\ensuremath{\bigcap}}}}


\newcommand{\QcirP}{\operatorname{\Q\mkern-2mu\odot\mkern-2mu\P}}
\newcommand{\subQcirP}{\operatorname{\Q \odot \P}}
\newcommand{\subQetacirP}{\operatorname{\Q^\eta \odot \P}}
\newcommand{\QcirtP}[1]{\Q\mkern-4mu\underset{\scriptscriptstyle{#1}} {\odot}\mkern-4mu\P}
\newcommand{\hbr}[1]{^{\scriptscriptstyle{(#1)}}}
\newcommand{\nohbr}[1]{^{#1}}

\newcommand{\hl}[1]{{\color{red} #1 }}
\DeclareMathOperator{\esssup}{ess  \sup}
\DeclareMathOperator{\essinf}{ess  \inf}

%\usepackage[color]{showkeys}
%\definecolor{refkey}{gray}{0.7}
%\definecolor{labelkey}{gray}{0.7}

% Use subfiles technique following https://www.overleaf.com/learn/latex/Multi-file_LaTeX_projects#The_subfiles_package
\usepackage{subfiles} % Best loaded last in the preamble

